MT-LENS: An all-in-one Toolkit for Better Machine Translation Evaluation

We introduce MT-LENS, a framework designed to evaluate Machine Translation (MT) systems across a variety of tasks, including translation quality, gender bias detection, added toxicity, and robustness to misspellings. While several toolkits have become very popular for benchmarking the capabilities of Large Language Models (LLMs), existing evaluation tools often lack the ability to thoroughly assess the diverse aspects of MT performance. MT-LENS addresses these limitations by extending the capabilities of LM-eval-harness for MT, supporting state-of-the-art datasets and a wide range of evaluation metrics. It also offers a user-friendly platform to compare systems and analyze translations with interactive visualizations. MT-LENS aims to broaden access to evaluation strategies that go beyond traditional translation quality evaluation, enabling researchers and engineers to better understand the performance of a NMT model and also easily measure system's biases.

==> tables/datasets.tex <==
\begin{table*}[h]
\centering
\small
\begin{tabularx}{\textwidth}{lllr}
\toprule
\textbf{Task} & \textbf{Dataset} & \textbf{Task name} &  \textbf{Languages}  \\
\midrule
General-MT & \floresdataset \cite{nllbteam2022language} & \{src\}\_\{tgt\}\_flores\_\{split\} & 200\\

& \textsc{NTREX-128} \cite{federmann-etal-2022-ntrex} & \{src\}\_\{tgt\}\_ntrex & 128\\

& \textsc{TATOEBA} \cite{tiedemann-2020-tatoeba} & \{src\}\_\{tgt\}\_tatoeba & 555 \\
& \textsc{NTEU} \cite{bie-etal-2020-neural} & \{src\}\_\{tgt\}\_nteu & 25 \\
\cdashlinelr{1-4}
Added Toxicity & \holisticbias \cite{smith-etal-2022-im} & \{src\}\_\{tgt\}\_\{axis\}\_hb & 1  \\
\cdashlinelr{1-4}
Gender Bias & \textsc{MuST-SHE} \cite{bentivogli-etal-2020-gender} & \{src\}\_\{tgt\}\_must\_she & 5  \\
& \textsc{MMHB} \cite{tan2024massivemultilingualholisticbias} & \{src\}\_\{tgt\}\_mmhb\_\{split\} & 7  \\
& \textsc{MT-GenEval} \cite{currey-etal-2022-mtgeneval} & \{src\}\_\{tgt\}\_geneval\_\{split\} &  8 \\
\cdashlinelr{1-4}
{\footnotesize Robustness to Character Noise} & \floresdataset devtest & \{src\}\_\{tgt\}\_perturbations & 200  \\
\bottomrule
\end{tabularx}
\caption{Machine translation datasets natively supported by {\mtlens} grouped by task type.}\label{table:datasets}
\end{table*}

==> tables/metrics.tex <==
\begin{table*}[ht]
\centering
\small
\begin{tabularx}{\textwidth}{XXX}
\toprule
\textbf{Type} & \textbf{Name} & \textbf{Implementation} \\
\midrule
Overlap Reference-based & \bleu\; \cite{papineni-etal-2002-bleu} & \texttt{SacreBLEU} \cite{post-2018-call} \\
& \ter\; \cite{snover-etal-2006-study} & \texttt{SacreBLEU} \\
& \chrf\; \cite{popovic-2015-chrf} & \texttt{SacreBLEU} \\
\cdashlinelr{1-3}
Neural Reference-based & \comet\; \cite{rei-etal-2022-comet} & \texttt{unbabel-comet} \cite{stewart-etal-2020-comet} \\
& \bleurt\; \cite{sellam-etal-2020-bleurt} & \texttt{transformers} \cite{wolf-etal-2020-transformers} \\
& \metricx & \texttt{metricx} \cite{juraska-etal-2023-metricx} \\
\cdashlinelr{1-3}
Neural Reference-based and error span & \xcomet\; \cite{guerreiro2023xcomet} & \texttt{unbabel-comet} \\
\cdashlinelr{1-3}
Quality estimation & \metricxqe\; & \texttt{metricx} \\
& \cometkiwi\; \cite{rei-etal-2022-cometkiwi} & \texttt{unbabel-comet} \\
\cdashlinelr{1-3}
Quality estimation and error span & \xcometqe\; & \texttt{unbabel-comet} \\
\cdashlinelr{1-3}
Word lists & {\etox} & \texttt{nllb} \cite{nllbteam2022language} \\
\cdashlinelr{1-3}
 Embedding-based & {\mutox} \cite{costa-jussa-etal-2024-mutox} & \texttt{seamless} \cite{communication2023seamlessmultilingualexpressivestreaming} \\
& {\detoxify} & \texttt{detoxify} \cite{detoxify} \\
\bottomrule
\end{tabularx}
\caption{Evaluation metrics supported by \mtlens.}\label{table:metrics}
\end{table*}

